RL Dreams: Policy Gradient Optimization for Score Distillation based 3D Generation

3D generation has rapidly accelerated in the past decade owing to the progress in the field of generative modeling. Score Distillation Sampling (SDS) based rendering has improved 3D asset generation to a great extent. Further, the recent work of Denoising Diffusion Policy Optimization (DDPO) demonstrates that the diffusion process is compatible with policy gradient methods and has been demonstrated to improve the 2D diffusion models using an aesthetic scoring function. We first show that this aesthetic scorer acts as a strong guide for a variety of SDS-based methods and demonstrates its effectiveness in text-to-3D synthesis. Further, we leverage the DDPO approach to improve the quality of the 3D rendering obtained from 2D diffusion models. Our approach, DDPO3D, employs the policy gradient method in tandem with aesthetic scoring. To the best of our knowledge, this is the first method that extends policy gradient methods to 3D score-based rendering and shows improvement across SDS-based methods such as DreamGaussian, which are currently driving research in text-to-3D synthesis. Our approach is compatible with score distillation-based methods, which would facilitate the integration of diverse reward functions into the generative process. Our project page can be accessed via https://ddpo3d.github.io.

==> sec/pipeline.tex <==
% Gradient Info
  
\tikzset {_c7g0c6va8/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_40i9w9w0o}{150bp}{rgb(0bp)=(0.65,0.81,0.87);
rgb(37.5bp)=(0.65,0.81,0.87);
rgb(62.5bp)=(0.14,0.33,0.54);
rgb(100bp)=(0.14,0.33,0.54)}
\tikzset{_40yph1pb7/.code = {\pgfsetadditionalshadetransform{\pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 } }}}
\pgfdeclarehorizontalshading{_w40wbwcvb} {150bp} {color(0bp)=(transparent!0);
color(37.5bp)=(transparent!0);
color(62.5bp)=(transparent!19);
color(100bp)=(transparent!19) } 
\pgfdeclarefading{_3fx1pk3ku}{\tikz \fill[shading=_w40wbwcvb,_40yph1pb7] (0,0) rectangle (50bp,50bp); } 

% Gradient Info
  
\tikzset {_qsy0ms9vw/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_9yj4nk0ah}{150bp}{rgb(0bp)=(0.6,0.85,1);
rgb(37.5bp)=(0.6,0.85,1);
rgb(62.478738512311665bp)=(0,0.5,0.5);
rgb(100bp)=(0,0.5,0.5)}
\tikzset{_r55n4vxze/.code = {\pgfsetadditionalshadetransform{\pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 } }}}
\pgfdeclarehorizontalshading{_renhgould} {150bp} {color(0bp)=(transparent!31);
color(37.5bp)=(transparent!31);
color(62.478738512311665bp)=(transparent!40);
color(100bp)=(transparent!40) } 
\pgfdeclarefading{_zsrsj3hb9}{\tikz \fill[shading=_renhgould,_r55n4vxze] (0,0) rectangle (50bp,50bp); } 

% Gradient Info
  
\tikzset {_w1fylciar/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{-198 bp } { 158.4 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_it4h3onfu}{\pgfpoint{160bp}{-128bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0.72,0.91,0.53);
rgb(400bp)=(0.72,0.91,0.53)}

% Gradient Info
  
\tikzset {_klrm1wnx0/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{-198 bp } { 158.4 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_1puwubb09}{\pgfpoint{160bp}{-128bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0.72,0.91,0.53);
rgb(400bp)=(0.72,0.91,0.53)}

% Gradient Info
  
\tikzset {_1nwq35bjk/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{-198 bp } { 158.4 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_p8uifga5g}{\pgfpoint{160bp}{-128bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0.72,0.91,0.53);
rgb(400bp)=(0.72,0.91,0.53)}

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_dhnbnzlnk}{
\makeatletter
\pgfdeclarepatternformonly[\mcRadius,\mcThickness,\mcSize]{_dhnbnzlnk}
{\pgfpoint{-0.5*\mcSize}{-0.5*\mcSize}}
{\pgfpoint{0.5*\mcSize}{0.5*\mcSize}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathcircle\pgfpointorigin{\mcRadius}
\pgfusepath{stroke}
}}
\makeatother

% Gradient Info
  
\tikzset {_6ss5krq40/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_47zy2hw7x}{150bp}{rgb(0bp)=(0.6,0.85,1);
rgb(37.5bp)=(0.6,0.85,1);
rgb(62.5bp)=(0,0.5,0.5);
rgb(100bp)=(0,0.5,0.5)}
\tikzset{_sm443wldo/.code = {\pgfsetadditionalshadetransform{\pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 } }}}
\pgfdeclarehorizontalshading{_l0nb5qizc} {150bp} {color(0bp)=(transparent!34);
color(37.5bp)=(transparent!34);
color(62.5bp)=(transparent!44.99999999999999);
color(100bp)=(transparent!44.99999999999999) } 
\pgfdeclarefading{_kave5ob0i}{\tikz \fill[shading=_l0nb5qizc,_sm443wldo] (0,0) rectangle (50bp,50bp); } 

% Gradient Info
  
\tikzset {_ablc6jrf7/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_ulbcw8twq}{150bp}{rgb(0bp)=(1,1,1);
rgb(37.5bp)=(1,1,1);
rgb(62.5bp)=(0.29,0.56,0.89);
rgb(100bp)=(0.29,0.56,0.89)}
\tikzset{_nzx90vihi/.code = {\pgfsetadditionalshadetransform{\pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 } }}}
\pgfdeclarehorizontalshading{_wp69ehssz} {150bp} {color(0bp)=(transparent!0);
color(37.5bp)=(transparent!0);
color(62.5bp)=(transparent!35);
color(100bp)=(transparent!35) } 
\pgfdeclarefading{_97gle6ahm}{\tikz \fill[shading=_wp69ehssz,_nzx90vihi] (0,0) rectangle (50bp,50bp); } 

% Gradient Info
  
\tikzset {_wapvt4307/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_iu6xd6hpy}{150bp}{rgb(0bp)=(1,1,1);
rgb(37.5bp)=(1,1,1);
rgb(62.5bp)=(0.82,0.92,0.98);
rgb(100bp)=(0.82,0.92,0.98)}

% Gradient Info
  
\tikzset {_vmmzhb1rl/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_kp72wfwnd}{150bp}{rgb(0bp)=(1,1,1);
rgb(37.5bp)=(1,1,1);
rgb(62.5bp)=(0.29,0.56,0.89);
rgb(100bp)=(0.29,0.56,0.89)}
\tikzset{_f6b5unhz7/.code = {\pgfsetadditionalshadetransform{\pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 } }}}
\pgfdeclarehorizontalshading{_hvd8nz494} {150bp} {color(0bp)=(transparent!0);
color(37.5bp)=(transparent!0);
color(62.5bp)=(transparent!32);
color(100bp)=(transparent!32) } 
\pgfdeclarefading{_f6rxjd6j2}{\tikz \fill[shading=_hvd8nz494,_f6b5unhz7] (0,0) rectangle (50bp,50bp); } 

% Gradient Info
  
\tikzset {_fwa3et6m2/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_nucytv99m}{150bp}{rgb(0bp)=(1,1,1);
rgb(37.5bp)=(1,1,1);
rgb(62.5bp)=(0.9,0.9,0.9);
rgb(100bp)=(0.9,0.9,0.9)}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Cube [id:dp08019308384615198] 
\path  [shading=_40i9w9w0o,_c7g0c6va8,path fading= _3fx1pk3ku ,fading transform={xshift=2}] (25,77.3) -- (43.3,59) -- (101.67,59) -- (101.67,101.7) -- (83.37,120) -- (25,120) -- cycle ; % for fading 
 \draw   (25,77.3) -- (43.3,59) -- (101.67,59) -- (101.67,101.7) -- (83.37,120) -- (25,120) -- cycle ; % for border 
 \draw   (101.67,59) -- (83.37,77.3) -- (25,77.3) ; \draw   (83.37,77.3) -- (83.37,120) ;
%Right Arrow [id:dp5314868353120741] 
\draw  [draw opacity=0][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.45 ] (215,75) -- (247.47,75) -- (247.47,65) -- (269.11,85) -- (247.47,105) -- (247.47,95) -- (215,95) -- cycle ;
%Shape: Rectangle [id:dp622323942068516] 
\draw  [draw opacity=0][shading=_9yj4nk0ah,_qsy0ms9vw,path fading= _zsrsj3hb9 ,fading transform={xshift=2}] (275,50) -- (345.67,50) -- (345.67,118) -- (275,118) -- cycle ;
%Straight Lines [id:da7658118237253138] 
\draw    (136.67,39) -- (106.67,136) ;
%Shape: Ellipse [id:dp020151608680414546] 
\draw  [draw opacity=0][shading=_it4h3onfu,_w1fylciar] (143.8,69.27) .. controls (143.8,65.2) and (151.53,61.9) .. (161.06,61.9) .. controls (170.59,61.9) and (178.31,65.2) .. (178.31,69.27) .. controls (178.31,73.35) and (170.59,76.65) .. (161.06,76.65) .. controls (151.53,76.65) and (143.8,73.35) .. (143.8,69.27) -- cycle ;
%Shape: Ellipse [id:dp5289938251981232] 
\draw  [draw opacity=0][shading=_1puwubb09,_klrm1wnx0] (132.36,113.39) .. controls (130.47,110.96) and (136.82,101.94) .. (146.55,93.25) .. controls (156.28,84.56) and (165.7,79.48) .. (167.59,81.91) .. controls (169.48,84.34) and (163.13,93.36) .. (153.4,102.05) .. controls (143.67,110.75) and (134.25,115.82) .. (132.36,113.39) -- cycle ;
%Shape: Ellipse [id:dp7402426249564] 
\draw  [draw opacity=0][shading=_p8uifga5g,_1nwq35bjk][line width=0.75]  (194.16,109.38) .. controls (189.19,109.05) and (185.8,97.8) .. (186.57,84.26) .. controls (187.35,70.71) and (192,59.99) .. (196.97,60.31) .. controls (201.93,60.64) and (205.33,71.89) .. (204.55,85.44) .. controls (203.78,98.99) and (199.12,109.71) .. (194.16,109.38) -- cycle ;
%Shape: Rectangle [id:dp5918887773757948] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.5 ][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.33 ] (209.56,164.41) -- (232.8,186.08) -- (210.08,210.44) -- (186.84,188.77) -- cycle ;
%Shape: Rectangle [id:dp5460854140792799] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.5 ][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.36 ] (191.99,158.28) -- (204.08,169.75) -- (191.7,182.81) -- (179.6,171.35) -- cycle ;
%Straight Lines [id:da002910460811637927] 
\draw    (183.11,143.33) -- (188,162) ;
%Straight Lines [id:da05697064028074483] 
\draw    (163.11,162.33) -- (185,167) ;
%Right Arrow [id:dp47999315722628055] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (353,79.38) -- (391.19,79.38) -- (391.19,74.38) -- (396.57,79.38) -- (391.19,84.38) -- (391.19,79.38) -- (353,79.38) -- cycle ;
%Shape: Rectangle [id:dp7824937237796805] 
\draw  [pattern=_dhnbnzlnk,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0.75pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (403,105) -- (473.67,105) -- (473.67,173) -- (403,173) -- cycle ;
%Shape: Rectangle [id:dp15314601942729666] 
\draw  [draw opacity=0][shading=_47zy2hw7x,_6ss5krq40,path fading= _kave5ob0i ,fading transform={xshift=2}] (400,10) -- (470.67,10) -- (470.67,78) -- (400,78) -- cycle ;
%Shape: Trapezoid [id:dp25309040438068076] 
\draw   (513.46,54.87) -- (553.39,67.13) -- (553.09,113.13) -- (513.01,124.87) -- cycle ;
%Shape: Trapezoid [id:dp8643627799027864] 
\draw   (596.31,124.96) -- (556.28,113.04) -- (556.19,67.04) -- (596.17,54.96) -- cycle ;
%Straight Lines [id:da23590596903979555] 
\draw    (550.11,45.33) -- (550.99,60.34) ;
\draw [shift={(551.11,62.33)}, rotate = 266.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da41414720562294804] 
\draw    (474.89,24.33) .. controls (514.49,-5.37) and (606.03,-0.76) .. (662.2,17.77) ;
\draw [shift={(663.89,18.33)}, rotate = 198.74] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp3099765615639878] 
\draw  [draw opacity=0][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.44 ] (668.78,139) -- (738.78,139) -- (738.78,193.33) -- (668.78,193.33) -- cycle ;
%Shape: Rectangle [id:dp12540065040108384] 
\draw  [draw opacity=0][shading=_ulbcw8twq,_ablc6jrf7,path fading= _97gle6ahm ,fading transform={xshift=2}] (604,58) -- (661.89,58) -- (661.89,119.33) -- (604,119.33) -- cycle ;
%Left Arrow [id:dp9318400392183388] 
\path  [shading=_iu6xd6hpy,_wapvt4307] (280.89,250) -- (309.14,230) -- (309.14,241.86) -- (737.14,241.86) -- (737.14,258.14) -- (309.14,258.14) -- (309.14,270) -- cycle ; % for fading 
 \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.27 ] (280.89,250) -- (309.14,230) -- (309.14,241.86) -- (737.14,241.86) -- (737.14,258.14) -- (309.14,258.14) -- (309.14,270) -- cycle ; % for border 

%Shape: Block Arc [id:dp9847659684901424] 
\draw   (568.04,91.82) .. controls (567.89,91.25) and (567.82,90.64) .. (567.83,90.01) .. controls (567.9,86.76) and (570.3,84.19) .. (573.18,84.28) .. controls (576.07,84.36) and (578.34,87.06) .. (578.27,90.31) .. controls (578.26,90.94) and (578.16,91.54) .. (577.98,92.11) -- (576.03,91.34) .. controls (576.12,90.99) and (576.18,90.63) .. (576.18,90.25) .. controls (576.23,88.15) and (574.87,86.41) .. (573.14,86.36) .. controls (571.41,86.31) and (569.97,87.97) .. (569.92,90.07) .. controls (569.91,90.45) and (569.95,90.82) .. (570.03,91.16) -- cycle ;
%Rounded Same Side Corner Rect [id:dp31524238821231143] 
\draw   (578.85,98.35) .. controls (578.84,99.18) and (578.15,99.84) .. (577.32,99.82) -- (568.23,99.63) .. controls (567.4,99.61) and (566.73,98.92) .. (566.75,98.09) -- (566.85,92.05) .. controls (566.85,92.05) and (566.85,92.05) .. (566.85,92.05) -- (578.95,92.31) .. controls (578.95,92.31) and (578.95,92.31) .. (578.95,92.31) -- cycle ;
%Shape: Trapezoid [id:dp7294603805975015] 
\draw   (513.46,127.87) -- (553.39,140.13) -- (553.09,186.13) -- (513.01,197.87) -- cycle ;
%Shape: Trapezoid [id:dp7306588945320491] 
\draw   (596.31,197.96) -- (556.28,186.04) -- (556.19,140.04) -- (596.17,127.96) -- cycle ;
%Shape: Block Arc [id:dp6785841373756001] 
\draw   (566.85,165.05) .. controls (566.5,164.57) and (566.21,164.02) .. (565.99,163.43) .. controls (564.89,160.37) and (566.2,157.12) .. (568.92,156.15) .. controls (571.64,155.19) and (574.73,156.89) .. (575.84,159.95) .. controls (576.05,160.54) and (576.18,161.14) .. (576.22,161.73) -- (574.12,161.71) .. controls (574.08,161.36) and (574,161) .. (573.87,160.64) .. controls (573.16,158.67) and (571.26,157.54) .. (569.63,158.12) .. controls (568,158.7) and (567.25,160.76) .. (567.96,162.73) .. controls (568.09,163.09) and (568.26,163.42) .. (568.46,163.72) -- cycle ;
%Rounded Same Side Corner Rect [id:dp05263697621671448] 
\draw   (578.85,171.35) .. controls (578.84,172.18) and (578.15,172.84) .. (577.32,172.82) -- (568.23,172.63) .. controls (567.4,172.61) and (566.73,171.92) .. (566.75,171.09) -- (566.85,165.05) .. controls (566.85,165.05) and (566.85,165.05) .. (566.85,165.05) -- (578.95,165.31) .. controls (578.95,165.31) and (578.95,165.31) .. (578.95,165.31) -- cycle ;
%Shape: Rectangle [id:dp8511382863700181] 
\draw  [draw opacity=0][shading=_kp72wfwnd,_vmmzhb1rl,path fading= _f6rxjd6j2 ,fading transform={xshift=2}] (604,134) -- (661.89,134) -- (661.89,195.33) -- (604,195.33) -- cycle ;
%Straight Lines [id:da2457513723050584] 
\draw    (475.95,79.86) -- (510.17,160.02) ;
\draw [shift={(510.95,161.86)}, rotate = 246.89] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1993063495044236] 
\draw    (475.95,79.86) -- (508.95,78.91) ;
\draw [shift={(510.95,78.86)}, rotate = 178.36] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da45883694002890585] 
\draw    (479.95,145.86) -- (509.98,91.61) ;
\draw [shift={(510.95,89.86)}, rotate = 118.97] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9535707105774187] 
\draw    (479.95,145.86) -- (509.18,160.94) ;
\draw [shift={(510.95,161.86)}, rotate = 207.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp48632088602488266] 
\draw  [draw opacity=0][fill={rgb, 255:red, 192; green, 53; blue, 53 }  ,fill opacity=0.45 ] (673.71,8.86) -- (740.52,8.86) -- (740.52,64) -- (673.71,64) -- cycle ;
\draw   (713.48,69.86) .. controls (729.44,87.08) and (745.41,97.41) .. (761.38,100.86) .. controls (745.41,104.3) and (729.44,114.63) .. (713.48,131.86) ;
%Rounded Rect [id:dp8365310208037162] 
\draw  [draw opacity=0][shading=_nucytv99m,_fwa3et6m2] (766.24,88.97) .. controls (766.24,83.46) and (770.7,79) .. (776.21,79) -- (830.08,79) .. controls (835.58,79) and (840.05,83.46) .. (840.05,88.97) -- (840.05,118.89) .. controls (840.05,124.39) and (835.58,128.86) .. (830.08,128.86) -- (776.21,128.86) .. controls (770.7,128.86) and (766.24,124.39) .. (766.24,118.89) -- cycle ;
%Straight Lines [id:da9841644796041713] 
\draw    (555.86,209) -- (554.97,194) ;
\draw [shift={(554.86,192)}, rotate = 86.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (40,91) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {NeRF};
% Text Node
\draw (123,121) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Gaussian Splatting};
% Text Node
\draw (217,79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Render};
% Text Node
\draw (190.7,181.81) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {camera};
% Text Node
\draw (292,79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {Image};
% Text Node
\draw (419,40) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {Image};
% Text Node
\draw (420.76,179) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {noise};
% Text Node
\draw (431.76,84) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {+};
% Text Node
\draw (506.38,30) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {"an image of a ..."};
% Text Node
\draw (528.38,9) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textbf{Prompt}}};
% Text Node
\draw (518,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {UNet};
% Text Node
\draw (677.78,147) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {{\footnotesize compute }\\{\footnotesize log-prob from}\\{\footnotesize  denoising step}};
% Text Node
\draw (517,159) node [anchor=north west][inner sep=0.75pt]   [align=left] {Unet};
% Text Node
\draw (687.29,16) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Aesthetic\\Scoring
\begin{undefined}
 Module
\end{undefined}
};
% Text Node
\draw (768.24,90) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Compute\\policy gradient};
% Text Node
\draw (417.73,247) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Backprop Policy Gradients with SDS gradients};
% Text Node
\draw (513.38,212) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {"an image of a ..."};
% Text Node
\draw (536.38,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textbf{Prompt}}};


\end{tikzpicture}
